BugListener: Identifying and Synthesizing Bug Reports from Collaborative Live Chats

In community-based software development, developers frequently rely on live-chatting to discuss emergent bugs/errors they encounter in daily development tasks. However, it remains a challenging task to accurately record such knowledge due to the noisy nature of interleaved dialogs in live chat data. In this paper, we first formulate the task of identifying and synthesizing bug reports from community live chats, and propose a novel approach, named BugListener, to address the challenges. Specifically, BugListener automates three sub-tasks: 1) Disentangle the dialogs from massive chat logs by using a Feed-Forward neural network; 2) Identify the bug-report dialogs from separated dialogs by modeling the original dialog to the graph-structured dialog and leveraging the graph neural network to learn the contextual information; 3) Synthesize the bug reports by utilizing the TextCNN model and Transfer Learning network to classify the sentences into three groups: observed behaviors (OB), expected behaviors (EB), and steps to reproduce the bug (SR). BugListener is evaluated on six open source projects. The results show that: for bug report identification, BugListener achieves the average F1 of 74.21%, improving the best baseline by 10.37%; and for bug report synthesis task, BugListener could classify the OB, EB, and SR sentences with the F1 of 67.37%, 87.14%, and 65.03%, improving the best baselines by 7.21%, 7.38%, 5.30%, respectively. A human evaluation also confirms the effectiveness of BugListener in generating relevant and accurate bug reports. These demonstrate the significant potential of applying BugListener in community-based software development, for promoting bug discovery and quality improvement.

==> sec/rw.tex <==
%\vspace{-0.3cm}
\section{Related Work}

\textbf{Identifying Bug Reports.}
Identifying bug reports from user feedback timely and precisely is vital for developers to update their applications. 
%The most related work to ours is the ISPY approach proposed by Shi et al \cite{}. ISPY can automatically extract issue-solution pairs from live chats by integrating natural language processing and deep learning techniques with customized enhancements. Although both studies mine valuable knowledge from live chats, our work differs from ISPY in the identified subject. ISPY targeted identifying resolved issues (such as installation/setup, build, or compile issues) and the corresponding solutions for future reuse, while our approach targets identifying unresolved bugs and synthesizing corresponding bug reports for improving quality timely. 
Many approaches have been proposed to identify bugs or problems from app reviews \cite{DBLP:conf/icse/0002S20,DBLP:conf/kbse/VuNPN15,DBLP:conf/kbse/VuPNN16,maalej2015bug,DBLP:journals/re/MaalejKNS16,DBLP:conf/icse/GaoZLK18,DBLP:conf/icse/GaoZD0ZLK19,DBLP:journals/tse/ScalabrinoBRPO19}, mailing lists \cite{DBLP:conf/kbse/SorboPVPCG15,DBLP:conf/icse/SorboPVPCG16}, and issue requests \cite{Huang2018Automating,DBLP:conf/icse/AryaWGC19,DBLP:conf/icsm/TerdchanakulHPM17,DBLP:journals/alr/Polpinij21,DBLP:conf/iwpc/PerezJUV21}.
For example, 
%Guo et al. \cite{DBLP:conf/icse/0002S20} proposed a method for extracting and synthesizing user reported mini stories regarding app problems from reviews. 
Vu et al. \cite{DBLP:conf/kbse/VuNPN15} detected emerging mobile bugs and trends by counting negative keywords based on Google Play. Since the single words might be ambiguous without contexts, their follow-up work \cite{DBLP:conf/kbse/VuPNN16} proposed a phrase-based clustering approach that relied on manual validation of part-of-speech (PoS) sequences. 
%Gao et al. \cite{DBLP:conf/icse/GaoZLK18} presented a topic labeling approach, named IDEA, to automatically detect bugs of current versions based on statistics of previous versions. 
%Due to the inborn limitations of topic modeling, such as the predefined topic numbers, their follow-up work \cite{DBLP:conf/icse/GaoZD0ZLK19} introduced DIVER which incorporated depth-first pattern mining with version and time-based comparisons.  
Maalej et al. \cite{maalej2015bug,DBLP:journals/re/MaalejKNS16} leveraged probabilistic techniques as well as text classification, natural language processing, and sentiment analysis techniques to classify app reviews into bug reports, feature requests, user experiences, and ratings. 
Scalabrino et al. \cite{DBLP:journals/tse/ScalabrinoBRPO19} developed CLAP to classify user reviews into bug reports, feature requests, and non-functional issues based on a random forest classifier.
%Arya et al. \cite{DBLP:conf/icse/AryaWGC19} classified 16 information types, including expected behavior, observed behavior, and new issues from issue discussion threads. 
Di Sorbo et al. \cite{DBLP:conf/kbse/SorboPVPCG15,DBLP:conf/icse/SorboPVPCG16} proposed a taxonomy of intentions to classify sentences in developer mailing lists into six categories: feature request, opinion asking, problem discovery, solution proposal, information seeking, and information giving. Although the taxonomy has been shown to be effective in analyzing development emails and user feedback from app reviews \cite{panichella2015how}, Huang et al. \cite{Huang2018Automating} found that it cannot be generalized to discussions in issue tracking systems, and they addressed the deficiencies of Di Sorbo et al.'s taxonomy by proposing a convolution neural network (CNN)-based approach. 
Our work differs from existing researches in that we focus on identifying bug reports from collaborative live chats, which post different challenges as chat messages are interleaved, unstructured, informal, and typically have insufficient labeled data than the previously analyzed documents.
%targets to automatically extract issues with their potential solutions (if exists) from community chats, complementing the existing studies on a novel source. In addition, our approach cannot only detect emerging issues in community chat, but also extract relevant solutions with resolved issues for reuse purposes, aiming to expedite the issue resolving process.

\textbf{Structuring or Synthesizing Bug Reports.}
A few efforts have been made to automatically structuring or synthesizing bug reports by utilizing heuristic rules \cite{bettenburg2008extracting,DBLP:conf/esem/DaviesR14,zimmermann2010makes,DBLP:conf/sigsoft/BettenburgJSWPZ08}. For example, keywords such as `error', `missing', and `does not work' were used to detect expected and observed behaviors \cite{zimmermann2010makes,DBLP:conf/esem/DaviesR14}.
As heuristic approaches often fail to capture the diverse discourse in bug reports, learning-based approaches have been proposed \cite{DBLP:conf/icsr/ZhaoMYZP19,DBLP:conf/sigsoft/ChaparroBLMMPPN19,DBLP:conf/kbse/ChenXYJCX20,song2020bee}.
%OB, EB, S2R
Song et al. \cite{song2020bee} proposed a tool that integrates three SVM models to identify the observed behavior, expected behavior, and S2R at the sentence level in bug reports.
%extract s2r from bug reports
Zhao et al. \cite{DBLP:conf/icsr/ZhaoMYZP19} proposed an SVM-based approach that can automatically extract the textual description of steps to reproduce (S2R) from bug reports for facilitating advance automated software issue diagnosis and test script reuse. 
%extract s2r from GUI interactions
Chaparro et al. \cite{DBLP:conf/sigsoft/ChaparroBLMMPPN19} proposed a  sequence-labeling-based approach that automatically assesses the quality of S2R in bug reports via matching the S2Rs to program states and GUI-level application interactions. By providing information such as steps missing in the report, their approach can benefit the automatic bug report synthesis for GUI-based systems. 
%generate title from bug-report body
Chen et al. \cite{DBLP:conf/kbse/ChenXYJCX20} proposed a seq2seq-based approach that can automatically generate titles regarding the textual bodies written in bug reports.
Most of these methods focus on structuring or synthesizing bug reports from textual descriptions that depicting bugs in a single-party style, while our 
approach targets to automatically structure and synthesize bug reports from multi-party conversations, complementing the existing studies on a novel resource.


% \textbf{Knowledge  Extraction from Collaborative Live Chats.}
% Recently, more and more work has realized that collaborative live chats play an increasingly significant role in software development, and collaborative live chats are a rich and untapped source for valuable information about the software system \cite{chatterjee2019exploratory,DBLP:conf/cscw/LinZSS16,DBLP:conf/msr/ChatterjeeDKP20}. 
% Several studies are focusing on extracting knowledge from collaborative live chats. 
% Chatterjee et al. \cite{DBLP:conf/icse/ChatterjeeDP21} 
% automatically collected opinion-based Q\&A from online developer chats, aiming to provide a valuable resource for developers in quickly getting insight about a specific development topic (e.g., What is the best Java library for parsing JSON?).
% Shi et al. \cite{DBLP:conf/icse/ShiXLWL020} proposed an approach to detect feature-request dialogues from developer chat messages via the deep siamese network.  
% %UIT 
% %Qu et al. \cite{InforSeek_User_Intent_Pred} utilized classic machine learning methods to perform user intent prediction with an average F1 of 0.67. 
% %user story
% Rodeghero et al. \cite{DBLP:conf/icse/RodegheroJAM17} presented a technique for automatically extracting information relevant to user stories from recorded conversations.
% % off-topic
% Chowdhury and Hindle \cite{chowdhury2015mining} filtered out off-topic discussions in programming IRC channels by engaging Stack Overflow discussions as positive examples and YouTube video comments. 
% The findings of previous work motivate the work presented in this paper. Our study is different from the previous work as we focus on identifying and synthesizing bug reports from massive chat messages that would be important and valuable information for software evolution.
% In addition, our work complements the existing studies on knowledge extraction from developer conversations.



==> tab/tab-rq2.tex <==


\begin{table*}[]
\caption{The performance achieved by different approaches for each project in intra-project validation}
\label{tab:rq2}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{\multirow{2}{*}{\diagbox{Approach\qquad}{Performance\qquad}}}   & \multicolumn{3}{c|}{AngularJS}                           & \multicolumn{3}{c|}{Bootstrap}                         & \multicolumn{3}{c|}{Chromium}                          \\ \cline{3-11} 
\multicolumn{2}{|c|}{}                           & Precision        & Recall           & F1               & Precision        & Recall           & F1               & Precision        & Recall           & F1               \\ \hline
\multirow{2}{*}{Our approach}        & FRMiner   & \textbf{90.28\%} & \textbf{89.73\%} & \textbf{90.00\%} & \textbf{86.28\%} & \textbf{88.78\%} & \textbf{87.52\%} & \textbf{89.00\%} & \textbf{87.00\%} & \textbf{88.00\%} \\ \cline{2-11} 
                                     & p-FRMiner & 31.71\%          & 54.17\%          & 40.00\%          & 50.00\%          & 47.80\%          & 48.98\%          & 14.00\%          & 44.00\%          & 20.00\%          \\ \hline
\multirow{2}{*}{Existing studies}    & CNC       & 7.70\%           & 44.44\%          & 13.13\%          & 16.38\%          & 34.21\%          & 22.13\%          & 9.56\%           & 67.00\%          & 16.73\%          \\ \cline{2-11} 
                                     & FRA       & 13.67\%          & 80.33\%          & 23.35\%          & 23.00\%          & 48.67\%          & 31.00\%          & 12.00\%          & {81.00\%} & 20.00\%          \\ \hline
\multirow{4}{*}{Text classification} & NB        & 20.00\%          & 27.67\%          & 22.33\%          & 25.67\%          & {62.00\%} & 36.00\%          & 14.33\%          & 44.33\%          & 21.00\%          \\ \cline{2-11} 
                                     & GBDT      & 36.00\%          & 22.33\%          & 27.33\%          & 41.67\%          & 35.67\%          & 38.33\%          & 9.33\%           & 7.33\%           & 8.00\%           \\ \cline{2-11} 
                                     & RF        & 52.67\%          & 11.00\%          & 16.33\%          & 57.00\%          & 29.00\%          & 38.33\%          & 0.00\%           & 0.00\%           & NA               \\ \cline{2-11} 
                                     & FT        & 23.33\%          & 5.33\%           & 8.67\%           & 57.67\%          & 29.00\%          & 38.33\%          & 38.00\%          & 9.10\%           & 15.00\%          \\ \hline
\end{tabular}
}
\end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}

==> tab/tab-rq3.tex <==


\begin{table*}[]
\caption{The performance achieved by different approaches for each project in cross-project validation}
\label{tab:rq3}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{}                                             & \multicolumn{3}{c|}{AngularJS}                                                                     & \multicolumn{3}{c|}{Bootstrap}                                                                   & \multicolumn{3}{c|}{Chromium}                                                                    \\ \cline{3-11} 
\multicolumn{2}{|c|}{\multirow{-2}{*}{\diagbox{Approach\qquad}{Performance\qquad}}}                    & Precision                      & Recall                         & F1                             & Precision                      & Recall                         & F1                             & Precision                      & Recall                         & F1                             \\ \hline
                                      & FRMiner                    & \textbf{85.23\%}               & \textbf{86.56\%}               & \textbf{85.89\%}               & \textbf{86.84\%}               & \textbf{85.89\%}               & \textbf{86.37\%}               & \textbf{85.87\%}               & \textbf{86.81\%}               & \textbf{86.34\%}               \\ \cline{2-11} 
\multirow{-2}{*}{Our approach}        & p-FRMiner                  & 31.03\%                        & 50.00\%                        & 38.30\%                        & 27.56\%                        & 69.08\%                        & 39.40\%                        & 16.00\%                        & 50.00\%                        & 24.24\%                        \\ \hline
                                      & {\color[HTML]{000000} CNC} & {\color[HTML]{000000} 7.70\%}  & {\color[HTML]{000000} 44.44\%} & {\color[HTML]{000000} 13.13\%} & {\color[HTML]{000000} 16.38\%} & {\color[HTML]{000000} 34.21\%} & {\color[HTML]{000000} 22.13\%} & {\color[HTML]{000000} 9.56\%}  & {\color[HTML]{000000} 67.00\%} & {\color[HTML]{000000} 16.73\%} \\ \cline{2-11} 
\multirow{-2}{*}{Existing studies}    & {\color[HTML]{000000} FRA} & {\color[HTML]{000000} 13.67\%} & {\color[HTML]{000000} 80.33\%} & {\color[HTML]{000000} 23.35\%} & {\color[HTML]{000000} 23.00\%} & {\color[HTML]{000000} 48.67\%} & {\color[HTML]{000000} 31.00\%} & {\color[HTML]{000000} 12.00\%} & {\color[HTML]{000000} 81.00\%} & {\color[HTML]{000000} 20.00\%} \\ \hline
                                      & NB                         & 16.00\%                        & 75.00\%                        & 26.00\%                        & 27.00\%                        & 36.00\%                        & 31.00\%                        & 7.00\%                         & 26.00\%                        & 12.00\%                        \\ \cline{2-11} 
                                      & GBDT                       & 18.00\%                        & 14.00\%                        & 16.00\%                        & 30.00\%                        & 11.00\%                        & 16.00\%                        & 20.00\%                        & 19.00\%                        & 19.00\%                        \\ \cline{2-11} 
                                      & RF                         & 28.00\%                        & 14.00\%                        & 19.00\%                        & 37.00\%                        & 9.00\%                         & 15.00\%                        & 12.00\%                        & 26.00\%                        & 16.00\%                        \\ \cline{2-11} 
\multirow{-4}{*}{Text classification} & FT                         & 32.00\%                        & 19.00\%                        & 24.00\%                        & 43.00\%                        & 13.00\%                        & 20.00\%                        & 19.00\%                        & 11.00\%                        & 14.00\%                        \\ \hline
\end{tabular}
}
\end{table*}



==> todo.tex <==
et al. 斜体
调整citation顺序
%更新例子，时间，头像，名字

bug-report dialog
Bee -> BEE
double check RQ2 baselines

in chronological order not in a chronological order

move link to ref

threat add data augment
future work add transfer learning 

